A Fine-Grained Approach for Automated Conversion of JUnit Assertions to English

Converting source or unit test code to English has been shown to improve the maintainability, understandability, and analysis of software and tests. Code summarizers identify important statements in the source/tests and convert them to easily understood English sentences using static analysis and NLP techniques. However, current test summarization approaches handle only a subset of the variation and customization allowed in the JUnit assert API (a critical component of test cases) which may affect the accuracy of conversions. In this paper, we present our work towards improving JUnit test summarization with a detailed process for converting a total of 45 unique JUnit assertions to English, including 37 previously-unhandled variations of the assertThat method. This process has also been implemented and released as the AssertConvert tool. Initial evaluations have shown that this tool generates English conversions that accurately represent a wide variety of assertion statements which could be used for code summarization or other NLP analyses.

==> codeconversionrules.tex <==
\subsection*{Converting Java Code to English}
\danielle{This section needs to be reformatted and reduced. Start with the generics that have the same rule.} 
In order to convert the `plain old Java' code found in JUnit test cases into understandable English, our approach firstly uses the \href{http://javadoc.io/doc/com.github.javaparser/javaparser-core/3.2.10}{Javaparser
  library} (version 3.2.10) AST-pasrsing library. This library has classes for all Java constructs, with different levels of granularity. 20 \textit{Statement} classes represent different multi-expression constructs such as for/if/while loops and blocks. \textit{Expression Statements} can be further broken down into 23 \textit{Expression} classes. In our approach, because JUnit tests typically don't include loops and blocks we focus on the expression classes, with class having its own set of conversion rules. Expressions are parsed \emph{recursively} and the natural language is combined using pre-defined templates. Below the rules for each of the \textit{Expression} classes are detailed. In some cases, the rules for multiple classes are the same (such as for generics). \danielle{Relevant sources for similar rule sets are McBurney \& McMillan, Sridhara, Zhang, and Panichella.}

\noindent{\textbf{ArrayAccessExpr}}

\begin{enumerate}
\item
  The parsing function is called recursively on the \emph{index
  expression} and the resulting \emph{index phrase} is stored.
\item
  The parsing function is called recursively on the \emph{name
  expression} and the resulting \emph{name phrase} is stored.
\end{enumerate}

The final phrase returned is: ``Index'' + \emph{index phrase} + " of " +
\emph{name phrase}.

\paragraph{{Example:}}

\texttt{myArray{[}0{]}} becomes ``Index 0 of my array''

\noindent{\textbf{ArrayCreationExpr}}

In this case, the final phrase returned is: ``new'' + \emph{camel case
split of array type} + " is created".

\hypertarget{example-1}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-1}}

\texttt{new\ String{[}{]}} becomes ``new string array is created''

\noindent\textbf{ArrayInitializerExpr}

\begin{enumerate}


\item
  For each value used to initialize the array, the parsing function is
  called recursively on the \emph{value expression} and the resulting
  \emph{value phrase} is stored.
\item
  The values are combined with " and ".
\end{enumerate}

The final phrase returned is ``initialized with'' + \emph{value phrase}
+ " and " \emph{value phrase}.

\hypertarget{example-2}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-2}}

\texttt{myArray\ =\ new\ int{[}{]}\ \{1,2\}} becomes ``new int array is
created initialized with 1 and 2'' (see \emph{ArrayCreationExpr} rules
also)

\noindent\textbf{AssignExpr}

\hypertarget{setup}{%
\paragraph{\texorpdfstring{\textbf{Setup}}{Setup}}\label{setup}}

For this type of expression, three pieces of information are identified
and separately parsed:

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{target
  expression} and the resulting \emph{target phrase} is stored.
\item
  The parsing function is called recursively on the \emph{value
  expression} and the resulting \emph{value phrase} is stored.
\item
  The \emph{operator} is stored
\end{enumerate}

\hypertarget{operator-parsing}{%
\paragraph{** Operator Parsing**}\label{operator-parsing}}

There are a number of ``operators'' that can be found in an assignment
expression (+,-,/,\emph{, etc.). For each, the english equivalent is
saved as the }operator phrase*. Example: \texttt{+} becomes ``plus'' and
\texttt{/} becomes ``divided by''.

The final phrase returned is: \emph{target phrase} + " " +
\emph{operator phrase} + " " + \emph{value phrase}.

\hypertarget{example-3}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-3}}

\texttt{myInt\ =\ 5} becomes ``my int equals 5'' (see \emph{NameExpr}
rules also)

\hypertarget{binaryexpr}{%
\subsubsection*{\texorpdfstring{\textbf{BinaryExpr}}{BinaryExpr}}\label{binaryexpr}}

\hypertarget{setup-1}{%
\paragraph{\texorpdfstring{\textbf{Setup}}{Setup}}\label{setup-1}}

Like with the AssignExpr this type of expression has three pieces of
information that are identified and separately parsed:

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{left
  expression} and the resulting \emph{LEFT side phrase} is stored.
\item
  The parsing function is called recursively on the \emph{right
  expression} and the resulting \emph{RIGHT side phrase} is stored.
\item
  The \emph{operator} is stored
\end{enumerate}

\hypertarget{operator-parsing-1}{%
\paragraph{** Operator Parsing**}\label{operator-parsing-1}}

There are a number of ``operators'' that can be found in a binary
expression (\&, \textbar{}\textbar{}, +, -, \textless{}, \textgreater{},
etc.). For each, the english equivalent is saved as the \emph{operator
phrase}. Example: \texttt{!} becomes ``not'' and \texttt{/} becomes
``divided by''.

The final phrase returned is: \emph{LEFT side phrase} + " " +
\emph{operator phrase} + " " + \emph{RIGHT side phrase}.

\hypertarget{example-4}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-4}}

\texttt{75\ /\ 3} becomes ``75 divided by 3''

\hypertarget{booleanliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{BooleanLiteralExpr}}{BooleanLiteralExpr}}\label{booleanliteralexpr}}

In this case, the string version of the boolean expression is returned.

\hypertarget{example-5}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-5}}

\texttt{true} is just ``true''

\hypertarget{castexpr}{%
\subsubsection*{\texorpdfstring{\textbf{CastExpr}}{CastExpr}}\label{castexpr}}

\begin{enumerate}


\item
  First, the parsing function is called recursively on the \emph{cast
  expression} and stored as the \emph{cast phrase}.
\item
  Next the \emph{camel case split} of the \emph{cast type} is stored.
\end{enumerate}

The final phrase returned is: \emph{cast phrase} + " as " + \emph{camel
case split cast type}.

\hypertarget{example-6}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-6}}

\texttt{(long)\ 15} becomes ``15 as long''

\hypertarget{charliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{CharLiteralExpr}}{CharLiteralExpr}}\label{charliteralexpr}}

In this case, the string version of the character expression is
returned.

\hypertarget{example-7}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-7}}

\texttt{\textquotesingle{}a\textquotesingle{}} becomes ``a''

\hypertarget{classexpr}{%
\subsubsection*{\texorpdfstring{\textbf{ClassExpr}}{ClassExpr}}\label{classexpr}}

In this case, the \emph{camel case split} of the class expression is
returned.

\hypertarget{example-8}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-8}}

\texttt{Object.class} becomes ``object class''

\hypertarget{conditionalexpr}{%
\subsubsection*{\texorpdfstring{\textbf{ConditionalExpr}}{ConditionalExpr}}\label{conditionalexpr}}

In this case, the parsing function is called recursively on three
components: \emph{condition expression}, \emph{else expression}, and
\emph{then expression} and the resulting phrases are stored.

The final phrase returned is: \emph{then phrase} + " if " +
\emph{condition phrase} + " otherwise " + \emph{else phrase}.

\hypertarget{example-9}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-9}}

\texttt{b==0?x:y} becomes ``x if b equals 0 otherwise y'' (see
\emph{NameExpr} rules also)

\hypertarget{doubleliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{DoubleLiteralExpr}}{DoubleLiteralExpr}}\label{doubleliteralexpr}}

In this case, the string version of the double is returned.

\hypertarget{example-10}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-10}}

\texttt{23958D} just becomes ``23958''

\hypertarget{enclosedexpr}{%
\subsubsection*{\texorpdfstring{\textbf{EnclosedExpr}}{EnclosedExpr}}\label{enclosedexpr}}

\textbf{Case 1: There is an \emph{inner expression}.}

In this case, the parsing function is called recursively on the
\emph{inner expression} and IF the inner expression is not the resulting
\emph{inner phrase} is stored.

\hypertarget{example-11}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-11}}

\texttt{(1\ +\ 1)} becomes ``1 plus 1'' (see \emph{BinaryExpr} rules
also)

\textbf{Case 2: There is NOT an \emph{inner expression}.}

In this case, the final phrase returnes is just empty parentheses.

\hypertarget{fieldaccessexpr}{%
\subsubsection*{\texorpdfstring{\textbf{FieldAccessExpr}}{FieldAccessExpr}}\label{fieldaccessexpr}}

In this case, the parsing function is called recursively on the
\emph{scope expression} and the resulting \emph{scope phrase} is stored
(what accessed the field).

The final phrase returned is \emph{camel case split field name} + " of "
+ \emph{scope phrase}.

\hypertarget{example-12}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-12}}

\texttt{user.loginPassword} becomes ``login password of user''

\hypertarget{instanceofexpr}{%
\subsubsection*{\texorpdfstring{\textbf{InstanceOfExpr}}{InstanceOfExpr}}\label{instanceofexpr}}

In this case, the parsing function is called recursively on the
\emph{identifier expression} and the resulting \emph{identifier phrase}
is stored.

The final phrase returned is \emph{identifier phrase} + " is class " +
\emph{camel case split class name}.

\hypertarget{example-13}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-13}}

\texttt{auth\ instance\ of\ AuthenticationManager} becomes ``auth is
class authentication manager''

\hypertarget{integerliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{IntegerLiteralExpr}}{IntegerLiteralExpr}}\label{integerliteralexpr}}

In this case, the string version of the integer is returned.

\hypertarget{example-14}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-14}}

\texttt{2} just becomes ``2''

\hypertarget{lambdaexpr}{%
\subsubsection*{\texorpdfstring{\textbf{LambdaExpr}}{LambdaExpr}}\label{lambdaexpr}}

\begin{enumerate}


\item
  The parsing function is called recursively on the parameters and the
  resulting \emph{parameter phrase} is stored.
\item
  For the expression on the right, the \emph{lambda body}, the parsing
  function is called recursively and the resulting \emph{body phrase} is
  stored.
\end{enumerate}

The final returned phrase is \emph{parameter phrase} + " becomes " +
\emph{body phrase}\ldots{}.

\hypertarget{example-15}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-15}}

\texttt{(a,\ b)\ -\textgreater{}\ a+b} becomes ``a and b become a plus
b''

\hypertarget{longliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{LongLiteralExpr}}{LongLiteralExpr}}\label{longliteralexpr}}

In this case, the string version of the long is returned.

\hypertarget{example-16}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-16}}

\texttt{99999999L} becomes ``99999999''

\hypertarget{methodcallexpr}{%
\subsubsection*{\texorpdfstring{\textbf{MethodCallExpr}}{MethodCallExpr}}\label{methodcallexpr}}

\hypertarget{setup-2}{%
\paragraph{\texorpdfstring{\textbf{Setup}}{Setup}}\label{setup-2}}

\begin{enumerate}


\item
  Get the name of the method call and split by camel case into
  String{[}{]}.
\item
  Get the Expression object for the caller of the method.
\item
  If the caller object is not null, the parsing function is called
  recursively (NameExpr) and the resulting \emph{caller phrase} is
  stored.
\end{enumerate}

\hypertarget{method-name-parsing-rules}{%
\paragraph{\texorpdfstring{\textbf{Method Name Parsing
Rules}}{Method Name Parsing Rules}}\label{method-name-parsing-rules}}

\textbf{Case 1: The method name begins with `get' AND the method name
contains more than one word}

The word ``get'' is removed and the final returned phrase is the
\emph{camel case split of the remaining words}.

\textbf{Example:} \texttt{getUserToken()} becomes ``get user token''

\textbf{Case 2: The method name is of length 1 AND the method name is a
verb OR he method name is of length 1 AND the caller contains the method
name}

In this case, the method name is ONLY a verb. Therefore, the parameters
provide essential context as to WHAT is being ``verbed''

\begin{enumerate}


\item
  Add the method name (the verb) to the final phrase.
\item
  If the method contains parameters, then the parsing function is called
  recursively on each parameter and the resulting \emph{parameter
  phrase} is appended to the final phrase.
\item
  If the parameter is another method call, its \emph{parameter phrase}
  is surrounded by parentheses to help with readability
\item
  If there is more than one parameter, they are connected with ``and''
\end{enumerate}

The final returned phrase is \emph{verb} + " " + \emph{parameter phrase}
+ " and " + \emph{parameter phrase}

\textbf{Example:}

\texttt{publish(message,author)} becomes ``publish message and author''
(assuming those objects are named after their type)

\textbf{Case 3: The method name is ``toString''}

In this case, the final returned phrase is \emph{caller phrase} + " as a
string."

\textbf{Example:}

\texttt{responseCode.toString()} becomes ``int response code as a
string''

\textbf{Case 4: The first two terms in method name are VERB NOUN
\emph{and} the verb is not ``is'' or ``get'' \emph{and} there is no
caller}

In this case, the final returned phrase is: NOUN + " is " + (past
tense)VERB + + \emph{camel case split of remaining words}

\textbf{Example:}

\texttt{publishArticle()} becomes ``article is published''

\textbf{Case 5: The first two terms in method name are VERB NOUN
\emph{and} the verb is not ``is'' or ``get'' \emph{and} there IS a
caller}

\begin{enumerate}


\item
  The verb is converted to past tense
\item
  The parsing function is called recursively on the caller and the
  resulting \emph{caller phrase} is stored.
\end{enumerate}

The final returned phrase is: NOUN + " is " + (past tense)VERB +
\emph{camel case split of remaining words} + ``by'' + \emph{caller
phrase}

\textbf{Example:}

\texttt{editor.publishArticle()} becomes ``article is published by
editor''

\textbf{Case 6: The first three terms in method name are VERB ADJECTIVE
NOUN \emph{and} the verb is not ``is'' or ``get'' \emph{and} there is no
caller}

In this case, the final returned phrase is: ADJECTIVE + " " + NOUN + "
is " + (past tense)VERB + + \emph{camel case split of remaining words}

\textbf{Example:}

\texttt{publishNewArticle()} becomes ``new article is published''

\textbf{Case 7: The first three terms in method name are VERB ADJECTIVE
NOUN \emph{and} the verb is not ``is'' or ``get'' \emph{and} there IS a
caller}

\begin{enumerate}


\item
  The verb is converted to past tense
\item
  The parsing function is called recursively on the caller and the
  resulting \emph{caller phrase} is stored.
\end{enumerate}

The final returned phrase is: ADJECTIVE + " " + NOUN + " is " + (past
tense)VERB + \emph{camel case split of remaining words} + " by" +
\emph{caller phrase}

\textbf{Example:}

\texttt{editor.publishNewArticleWhenDone()} becomes ``new article is
published when done by editor''

**Case 8: The first term in method name ``is'' and the second term is a
verb In this case, the same rules as for cases 4-7 are followed
(template formats for NOUN, VERB, ADJECTIVE order), but the ``is'' term
in the template is not repeated. In this case, it it \emph{expected}
that the verb is already past tense.

\textbf{Example:}

\texttt{article.isSentToEditor()} becomes ``article is sent to editor''

Case 9: The same format of cases 5, 7, and 8 is followed, however, in
this case the caller starts with the word with. In this case, we the
final returned phrase is like that of 5, 7, and 9, but does not include
``by'' before the caller.

\textbf{Other Cases}

In any other case, the final returne phrase is \emph{caller phrase} +
\emph{camel case split of method name}

\textbf{Example:} \texttt{authman.checkCredentials(user,pass)} becomes
``auth manager check credentials''

\hypertarget{methodreferenceexpr}{%
\subsubsection*{\texorpdfstring{\textbf{MethodReferenceExpr}}{MethodReferenceExpr}}\label{methodreferenceexpr}}

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{scope
  expression} and the resulting \emph{scope phrase} is stored (what
  accessed the method).
\item
  The \emph{identifier} is stored
\item
  If the identifier is ``new'', the final phrase returned is: ``new'' +
  \emph{scope phrase} + " is created."
\item
  If the identifier is anything else, the final phrase returned is:
  \emph{scope phrase} + " " + \emph{identifier}.
\end{enumerate}

\#\#\#\#\textbf{Example:}\#\#\#\# \texttt{System.out::println;} becomes
``system out println''

\hypertarget{nameexpr}{%
\subsubsection*{\texorpdfstring{\textbf{NameExpr}}{NameExpr}}\label{nameexpr}}

The idea in this case is that, generally, the Type of the object is more
descriptive than its name. However, we don't want to assume that in all
cases, so we look at both and use a set of checks to see which is more
descriptive.

\hypertarget{setup-3}{%
\paragraph{\texorpdfstring{\textbf{Setup}}{Setup}}\label{setup-3}}

\begin{enumerate}


\item
  Store the \emph{camel case split} of the NameExpr as the \emph{name
  phrase}
\item
  Get the the \emph{name type} using the ObjectTypeSolver, and if so,
  get the ``base name'' by only taking the last part of the fully
  qualified type (split by ``.'' and take last piece). Example:
  \texttt{org.springframework.security.config.annotation.authentication.configuration.AuthenticationConfiguration}
  becomes \texttt{AuthenticationConfiguration}.
\item
  If the full \emph{name type} cannot be found, use the ``failed
  symbol'' from JavaSymbolSolver, which is usually the base type anyway.
\item
  If the ``failed symbol'' is also null, the \emph{name type} is set to
  null
\item
  If the \emph{name type} is null, the \emph{type phrase} is also set to
  null
\end{enumerate}

\textbf{Case 1: \emph{Type Phrase} is NOT NULL}

\begin{enumerate}


\item
  The \emph{type phrase} is set as the \emph{camel case split of the
  type}
\item
  If the \emph{type phrase} is ``boolean'', then the final returned
  phrase is just the \emph{name phrase}. \textbf{Example:}
  \texttt{boolean\ didItFail} becomes ``did it fail''
\item
  If the \emph{type phrase} is a numeric primitive (int, double, float,
  long), then the final returned phrase is \emph{type phrase} + " " +
  \emph{name phrase}. \textbf{Example:} \texttt{int\ response} becomes
  ``int response''
\item
  If the \emph{name phrase} is longer than the \emph{type phrase} AND
  \emph{includes} the ENTIRE type, then the final returned phrase is
  just the \emph{name phrase} \textbf{Example:}
  \texttt{Token\ userToken} becomes ``user token''
\item
  In all other cases, the final returned phrase is just the \emph{type
  phrase}
\end{enumerate}

\textbf{Case 2: \emph{Type Phrase} is NULL}

In this case, return just the \emph{camel case split of the name
phrase}. This happens if the ObjectTypeSolver fails to identify the
type.

\hypertarget{example-17}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-17}}

\texttt{myVariable} becomes ``my variable''

\hypertarget{nullliteralexpr}{%
\subsubsection*{\texorpdfstring{\textbf{NullLiteralExpr}}{NullLiteralExpr}}\label{nullliteralexpr}}

In this case, the phrase ``NULL'' is returned.

\hypertarget{objectcreationexpr}{%
\subsubsection*{\texorpdfstring{\textbf{ObjectCreationExpr}}{ObjectCreationExpr}}\label{objectcreationexpr}}

\begin{enumerate}


\item
  First, the term ``new'' is first prepended to the \emph{camel case
  split} of the \emph{object type}.
\item
  Next, The parsing function is called recursively on the
  \emph{parameter expressions} and the result is appended to the phrase.
\item
  Multiple parameters are combined using " and "
\end{enumerate}

The final returned phrase is: ``new'' + \emph{camel case split object
type} + \emph{parameter phrase} + " and " \emph{parameter phrase}.

\hypertarget{example-18}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-18}}

\texttt{ServerConfiguration\ conf\ =\ new\ ServerConfiguration(fileA)}
becomes ``new server configuration conf is set as new server
configuration with file'' (see \emph{VariableDeclarationExpr},
\emph{MethodCallExpr} and \emph{NameExpr} rules also)

\hypertarget{stringliteralexpr-string-literalstringvalueexpr}{%
\subsubsection*{\texorpdfstring{\textbf{StringLiteralExpr, String, \&
LiteralStringValueExpr}}{StringLiteralExpr, String, \& LiteralStringValueExpr}}\label{stringliteralexpr-string-literalstringvalueexpr}}

In this case, the word ``string'' is returned, not the actual value of
the string. This is because some strings can be long and unintelligible,
and through experimentation it was found that including them made the
summaries less comprehensible.

\hypertarget{superexpr}{%
\subsubsection*{\texorpdfstring{\textbf{SuperExpr}}{SuperExpr}}\label{superexpr}}

\textbf{Case 1: There is a class expression within the `super'
expression}

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{class
  expression} and the resulting \emph{class phrase} is stored.
\item
  The final phrase returned is: ``super of'' + \emph{class phrase}.
\end{enumerate}

\hypertarget{example-19}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-19}}

\texttt{World.super} becomes ``super of world''

\textbf{Case 2: There is NOT a class expression with the `super'
expression} 1. The final phrase returned is just " super ".

\hypertarget{thisexpr}{%
\subsubsection*{\texorpdfstring{\textbf{ThisExpr}}{ThisExpr}}\label{thisexpr}}

\textbf{Case 1: There is a class expression within the `this'
expression}

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{class
  expression} and the resulting \emph{class phrase} is stored.
\item
  The final phrase returned is: \emph{class phrase} + \emph{camel case
  split of the `this' expression}
\end{enumerate}

\hypertarget{example-20}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-20}}

\texttt{World.class.this.greet()} becomes ``world class this greet''

\textbf{Case 2: There is NOT a class expression with the `this'
expression} 1. The final phrase returned is the \emph{camel case split
of the `this' expression}

\hypertarget{example-21}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-21}}

\texttt{World.this.greet()} becomes ``world this greet''

\hypertarget{typeexpr}{%
\subsubsection*{\texorpdfstring{\textbf{TypeExpr}}{TypeExpr}}\label{typeexpr}}

\begin{enumerate}


\item
  If the type expression contains the word ``boolean'', the final phrase
  returned is nothing ("").
\item
  If the type expression does NOT contain the word ``boolean'', the
  final phrase returned is: ``type'' + \emph{camel case split of type}.
\end{enumerate}

\hypertarget{example-22}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-22}}

\texttt{AuthManager} becomes ``type auth manager''

\hypertarget{unaryexpr}{%
\subsubsection*{\texorpdfstring{\textbf{UnaryExpr}}{UnaryExpr}}\label{unaryexpr}}

Simialrly to the BinaryExpr, the major components are the
\emph{expression} and the \emph{operator}, except now there is no
left/right sides to combine.

Instead,

\begin{enumerate}


\item
  The parsing function is called recursively on the \emph{expression}
  and the resulting \emph{expression phrase} is stored.
\item
  There are a number of ``operators'' that can be found in a unary
  expression (++, --, etc.). For each, the english equivalent is saved
  as the \emph{operator phrase}. Example: \texttt{-\/-} becomes
  \texttt{minus\ ƒ1} and \texttt{++} becomes \texttt{plus\ 1}.
\end{enumerate}

The final phrase returned is the combination of the \emph{operator
phrase} and the \emph{expression phrase}, the order of which depends on
the operator. Example ``positive'' goes before the expression, but
\texttt{-1} goes after.

\hypertarget{example-23}{%
\paragraph{\texorpdfstring{\textbf{Example:}}{Example:}}\label{example-23}}

\texttt{myVar++} becomes ``int my var plus 1''

\hypertarget{variabledeclarationexpr}{%
\subsubsection*{\texorpdfstring{\textbf{VariableDeclarationExpr}}{VariableDeclarationExpr}}\label{variabledeclarationexpr}}

\hypertarget{setup-4}{%
\paragraph{\texorpdfstring{\textbf{Setup}}{Setup}}\label{setup-4}}

First, a list of variables is stored.

For each variable found,

\begin{enumerate}


\item
  The \emph{type phrase} is stored as a camel-case split string.
\item
  The \emph{name phrase} is stored as a camel-case split string.
\end{enumerate}

\hypertarget{building-variable-phrase}{%
\paragraph{\texorpdfstring{\textbf{Building Variable
Phrase}}{Building Variable Phrase}}\label{building-variable-phrase}}

\begin{enumerate}


\item
  If the \emph{type phrase} EQUALS the \emph{name phrase}, the final
  phrase for the variable is JUST the \emph{type phrase}.
  \textbf{Example}: \texttt{String\ string} becomes ``string''
\item
  If the \emph{type phrase} DOES NOT EQUAL the \emph{name phrase}, the
  final phrase for the variable is: \emph{type phrase} + " " +
  \emph{name phrase}. \textbf{Example}: \texttt{AuthManager\ myAuth}
  becomes ``auth manager my auth''
\item
  If there is an initializer, the parsing function is called recursively
  on the \emph{initializer expression} and the final phrase for the
  variable is \emph{type phrase + " equals" + }initializer phrase*
  \textbf{Example}:
  \texttt{SessionManager\ sess\ =\ new\ Session\ Manager()} becomes
  ``session manager equals new session manager''
\item
  Multiple variables are connected using " and ".
\end{enumerate}

\hypertarget{other-rules-for-readability}{%
\subsubsection*{\texorpdfstring{\textbf{Other Rules for
Readability}}{Other Rules for Readability}}\label{other-rules-for-readability}}

\begin{enumerate}


\item
  If the final phrase contains "\_``s or''."s remove these and replace
  them with spaces.
\item
  Replace any repetitive phrases, such as ``string plus string plus
  string'' with ``string plus strings''.
\end{enumerate}
